Muon Collider Forum Report

A multi-TeV muon collider offers a spectacular opportunity in the direct exploration of the energy frontier. Offering a combination of unprecedented energy collisions in a comparatively clean leptonic environment, a high energy muon collider has the unique potential to provide both precision measurements and the highest energy reach in one machine that cannot be paralleled by any currently available technology. The topic generated a lot of excitement in Snowmass meetings and continues to attract a large number of supporters, including many from the early career community. In light of this very strong interest within the US particle physics community, Snowmass Energy, Theory and Accelerator Frontiers created a cross-frontier Muon Collider Forum in November of 2020. The Forum has been meeting on a monthly basis and organized several topical workshops dedicated to physics, accelerator technology, and detector R&D. Findings of the Forum are summarized in this report.

==> muc-refs <==
%% Recent review on current and future accelerators
@article{Shiltsev:2019rfl,
    author = "Shiltsev, Vladimir and Zimmermann, Frank",
    title = "{Modern and Future Colliders}",
    eprint = "2003.09084",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "FERMILAB-PUB-19-481-AD-APC",
    doi = "10.1103/RevModPhys.93.015006",
    journal = "Rev. Mod. Phys.",
    volume = "93",
    pages = "015006",
    year = "2021"
}

%% Muon collider motivation
@article{Long:2020wfp,
    author = "Long, K. and Lucchesi, D. and Palmer, M. and Pastrone, N. and Schulte, D. and Shiltsev, V.",
    title = "{Muon colliders to expand frontiers of particle physics}",
    eprint = "2007.15684",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "FERMILAB-PUB-20-366-AD-APC",
    doi = "10.1038/s41567-020-01130-x",
    journal = "Nature Phys.",
    volume = "17",
    number = "3",
    pages = "289--292",
    year = "2021"
}

@article{Costantini:2020stv,
    author = "Costantini, Antonio and De Lillo, Federico and Maltoni, Fabio and Mantani, Luca and Mattelaer, Olivier and Ruiz, Richard and Zhao, Xiaoran",
    title = "{Vector boson fusion at multi-TeV muon colliders}",
    eprint = "2005.10289",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CP3-20-20, MCNET-20-12, VBSCAN-PUB-03-20",
    doi = "10.1007/JHEP09(2020)080",
    journal = "JHEP",
    volume = "09",
    pages = "080",
    year = "2020"
}

@article{AlAli:2021let,
    author = "Al Ali, Hind and others",
    title = "{The Muon Smasher's Guide}",
    eprint = "2103.14043",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2021"
}

@article{Han:2020uak,
    author = "Han, Tao and Liu, Zhen and Wang, Lian-Tao and Wang, Xing",
    title = "{WIMPs at High Energy Muon Colliders}",
    eprint = "2009.11287",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC 2009",
    doi = "10.1103/PhysRevD.103.075004",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "7",
    pages = "075004",
    year = "2021"
}

@article{Capdevilla:2021rwo,
    author = "Capdevilla, Rodolfo and Curtin, David and Kahn, Yonatan and Krnjaic, Gordan",
    title = "{No-lose theorem for discovering the new physics of (g-2)\ensuremath{\mu} at muon colliders}",
    eprint = "2101.10334",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-21-012-T",
    doi = "10.1103/PhysRevD.105.015028",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "1",
    pages = "015028",
    year = "2022"
}

@inproceedings{Alexahin:2013vla,
    author = "Alexahin, Yuri and others",
    title = "{The Case for a Muon Collider Higgs Factory}",
    booktitle = "{Community Summer Study 2013}: {Snowmass on the Mississippi}",
    eprint = "1307.6129",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-13-284-T",
    month = "7",
    year = "2013"
}



%%% Muon collider: historic papers
@article{Ankenbrandt:1999cta,
    author = "Ankenbrandt, Charles M. and others",
    title = "{Status of muon collider research and development and future plans}",
    eprint = "physics/9901022",
    archivePrefix = "arXiv",
    reportNumber = "BNL-65623, FERMILAB-PUB-98-179, LBNL-41935, LBL-41935",
    doi = "10.1103/PhysRevSTAB.2.081001",
    journal = "Phys. Rev. ST Accel. Beams",
    volume = "2",
    pages = "081001",
    year = "1999"
}

@article{Neuffer:1994bt,
    author = "Neuffer, David V. and Palmer, Robert B.",
    title = "{A High-Energy High-Luminosity $\mu^+ - \mu^-$ Collider}",
    reportNumber = "BNL-61267, CEBAF-PR-94-30",
    journal = "Conf. Proc. C",
    volume = "940627",
    pages = "52--54",
    year = "1995"
}

@article{Foster:1995ru,
    author = "Foster, G. William and Mokhov, Nikolai V.",
    editor = "Cline, D. B.",
    title = "{Backgrounds and detector performance at a 2 $\times$2 TeV $\mu^+ \mu^-$ collider}",
    reportNumber = "FERMILAB-CONF-95-037",
    doi = "10.1063/1.49354",
    journal = "AIP Conf. Proc.",
    volume = "352",
    pages = "178--190",
    year = "1996"
}
@article{Gallardo:1996aa,
    author = "Gallardo, J. C. and others",
    title = "{$\mu^+ \mu^-$ Collider: Feasibility Study}",
    reportNumber = "SLAC-R-988, BNL-52503, FERMILAB-CONF-96-092, LBL-38946, LBNL-38946",
    journal = "eConf",
    volume = "C960625",
    pages = "R4",
    year = "1996"
}

@article{Palmer:1996gs,
    author = "Palmer, R. and others",
    editor = "Cline, D. B.",
    title = "{Muon collider design}",
    eprint = "acc-phys/9604001",
    archivePrefix = "arXiv",
    reportNumber = "BNL-62949, SLAC-PUB-9921",
    doi = "10.1016/0920-5632(96)00417-3",
    journal = "Nucl. Phys. B Proc. Suppl.",
    volume = "51",
    pages = "61--84",
    year = "1996"
}

@article{Snopok:2007vyn,
    author = "Snopok, Pavel and Berz, Martin and Johnstone, Carol",
    editor = "Petit-Jean-Genaz, C.",
    title = "{A New Lattice Design for a 1.5-TeV CoM Muon Collider Consistent with the Tevatron Tunnel}",
    reportNumber = "FERMILAB-CONF-07-805-AD, PAC07-THPAN109",
    doi = "10.1109/PAC.2007.4440466",
    journal = "Conf. Proc. C",
    volume = "070625",
    pages = "3483",
    year = "2007"
}

@inproceedings{Alexahin:2013ojp,
    author = "Alexahin, Yuri and others",
    title = "{Muon Collider Higgs Factory for Snowmass 2013}",
    booktitle = "{Community Summer Study 2013}: {Snowmass on the Mississippi}",
    eprint = "1308.2143",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-13-245-T",
    month = "8",
    year = "2013"
}

@article{Alexahin:2012zzc,
    author = "Alexahin, Y. and Gianfelice-Wendt, E.",
    editor = "Suller, Vic",
    title = "{A 3 TeV Muon Collider Lattice Design}",
    reportNumber = "FERMILAB-CONF-12-184-APC, IPAC-2012-TUPPC041",
    journal = "Conf. Proc. C",
    volume = "1205201",
    pages = "1254--1256",
    year = "2012"
}

%%% Past performance studies
@article{muc-perf-2020,
   title={Detector and Physics Performance at a Muon Collider},
   volume={15},
   ISSN={1748-0221},
   url={http://dx.doi.org/10.1088/1748-0221/15/05/P05001},
   DOI={10.1088/1748-0221/15/05/p05001},
   number={05},
   journal={Journal of Instrumentation},
   publisher={IOP Publishing},
   author={Bartosik, N. and Bertolin, A. and Buonincontri, L. and Casarsa, M. and Collamati, F. and Ferrari, A. and Ferrari, A. and Gianelle, A. and Lucchesi, D. and Mokhov, N. and et al.},
   year={2020},
   month={May},
   pages={P05001–P05001}
}

%% BIB past studies
@article{Mokhov:1996tq,
    author = "Mokhov, N. V. and Striganov, S. I.",
    editor = "Gallardo, J. C.",
    title = "{Simulation of backgrounds in detectors and energy deposition in superconducting magnets at $\mu^{+}\mu^-$ colliders}",
    reportNumber = "FERMILAB-CONF-96-011",
    doi = "10.1063/1.50907",
    journal = "AIP Conf. Proc.",
    volume = "372",
    number = "1",
    pages = "234--256",
    year = "1996"
}

@article{Mokhov:2011zzd,
    author = "Mokhov, N. V. and Striganov, S. I.",
    editor = "Liu, Ted",
    title = "{Detector Background at Muon Colliders}",
    eprint = "1204.6721",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-PUB-11-483-APC",
    doi = "10.1016/j.phpro.2012.03.761",
    journal = "Phys. Procedia",
    volume = "37",
    pages = "2015--2022",
    year = "2012"
}

@article{Collamati:2021sbv,
    author = "Collamati, Francesco and Curatolo, Camilla and Lucchesi, Donatella and Mereghetti, Alessio and Mokhov, Nikolai and Palmer, Mark and Sala, Paola",
    title = "{Advanced assessment of beam-induced background at a muon collider}",
    eprint = "2105.09116",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "FERMILAB-PUB-21-345-AD
",
    doi = "10.1088/1748-0221/16/11/P11009",
    journal = "JINST",
    volume = "16",
    number = "11",
    pages = "P11009",
    year = "2021"
}

%%% Other physics prospects papers
@article{Buttazzo:2018qqp,
    author = "Buttazzo, Dario and Redigolo, Diego and Sala, Filippo and Tesi, Andrea",
    title = "{Fusing Vectors into Scalars at High Energy Lepton Colliders}",
    eprint = "1807.04743",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 18-116, DESY-18-116",
    doi = "10.1007/JHEP11(2018)144",
    journal = "JHEP",
    volume = "11",
    pages = "144",
    year = "2018"
}

@article{DiLuzio:2018jwd,
    author = {Di Luzio, Luca and Gr\"ober, Ramona and Panico, Giuliano},
    title = "{Probing new electroweak states via precision measurements at the LHC and future colliders}",
    eprint = "1810.10993",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "HU-EP-18/30, DESY 18-184, DESY-18-184",
    doi = "10.1007/JHEP01(2019)011",
    journal = "JHEP",
    volume = "01",
    pages = "011",
    year = "2019"
}

@article{Franceschini:2021dxn,
    author = "Franceschini, Roberto",
    title = "{High(est) energy lepton colliders}",
    doi = "10.1142/S0217751X21420161",
    journal = "Int. J. Mod. Phys. A",
    volume = "36",
    number = "22",
    pages = "2142016",
    year = "2021"
}

@article{Chiesa:2020awd,
    author = "Chiesa, M. and Maltoni, F. and Mantani, L. and Mele, B. and Piccinini, F. and Zhao, X.",
    title = "{Measuring the quartic Higgs self-coupling at a multi-TeV muon collider}",
    eprint = "2003.13628",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CP3-20-15, LAPTH-013/20, MCnet-20-12",
    doi = "10.1007/JHEP09(2020)098",
    journal = "JHEP",
    volume = "09",
    pages = "098",
    year = "2020"
}

@article{Han:2020pif,
    author = "Han, T. and Liu, D. and Low, I. and Wang, X.",
    title = "{Electroweak Couplings of the Higgs Boson at a Multi-TeV Muon Collider}",
    eprint = "2008.12204",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.013002",
    journal = "Phys. Rev. D",
    volume = "103",
    pages = "013002",
    year = "2021"
}

@article{Buttazzo:2020uzc,
    author = "Buttazzo, D. and Franceschini, R. and Wulzer, A.",
    title = "{Two Paths Towards Precision at a Very High Energy Lepton Collider}",
    eprint = "2012.11555",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-216",
    month = "12",
    year = "2020"
}

@article{Kalinowski:2020rmb,
    author = "Kalinowski, Jan and Robens, Tania and Sokolowska, Dorota and Zarnecki, Aleksander Filip",
    title = "{IDM Benchmarks for the LHC and Future Colliders}",
    eprint = "2012.14818",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "RBI-ThPhys-2020-55",
    doi = "10.3390/sym13060991",
    journal = "Symmetry",
    volume = "13",
    number = "6",
    pages = "991",
    year = "2021"
}

@article{Capdevilla:2020qel,
    author = "Capdevilla, R. and Curtin, D. and Kahn, Y. and Krnjaic, G.",
    title = "{A Guaranteed Discovery at Future Muon Colliders}",
    eprint = "2006.16277",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-20-290-T",
    month = "6",
    year = "2020"
}

@article{Buttazzo:2020eyl,
    author = "Buttazzo, D. and Paradisi, P.",
    title = "{Probing the muon g-2 anomaly at a Muon Collider}",
    eprint = "2012.02769",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "12",
    year = "2020"
}

@article{Yin:2020afe,
    author = "Yin, W. and Yamaguchi, M.",
    title = "{Muon $g-2$ at multi-TeV muon collider}",
    eprint = "2012.03928",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "12",
    year = "2020"
}

@article{Huang:2021nkl,
    author = "Huang, Guo-yuan and Queiroz, Farinaldo S. and Rodejohann, Werner",
    title = "{Gauged $L^{}_{\mu}{-}L^{}_{\tau}$ at a muon collider}",
    eprint = "2101.04956",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.095005",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "9",
    pages = "095005",
    year = "2021"
}

@article{Huang:2021nkl,
    author = "Huang, G.-Y. and Queiroz, F. S. and Rodejohann, W.",
    title = "{Gauged $L^{}_{\mu}{-}L^{}_{\tau}$ at a muon collider}",
    eprint = "2101.04956",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "1",
    year = "2021"
}

@article{Bartosik:2020xwr,
	Archiveprefix = {arXiv},
	Author = {Bartosik, Nazar and others},
	Doi = {10.1088/1748-0221/15/05/P05001},
	Eprint = {2001.04431},
	Journal = {JINST},
	Number = {05},
	Pages = {P05001},
	Primaryclass = {hep-ex},
	Reportnumber = {FERMILAB-PUB-20-014-AD},
	Title = {{Detector and Physics Performance at a Muon Collider}},
	Volume = {15},
	Year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1088/1748-0221/15/05/P05001}
}
	
@article{Liu:2021jyc,
     author = "Liu, Wei and Xie, Ke-Pan",
     title = "{Probing electroweak phase transition with multi-TeV muon colliders and gravitational waves}",
     eprint = "2101.10469",
     archivePrefix = "arXiv",
     primaryClass = "hep-ph",
     doi = "10.1007/JHEP04(2021)015",
     journal = "JHEP",
     volume = "04",
     pages = "015",
     year = "2021"
 }

@article{Chen:2021rnl,
    author = "Chen, N. and Wang, B. and Yao, C.-Y.",
    title = "{The collider tests of a leptophilic scalar for the anomalous magnetic moments}",
    eprint = "2102.05619",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "2",
    year = "2021"
}

@article{Ruhdorfer:2019utl,
    author = "Ruhdorfer, Maximilian and Salvioni, Ennio and Weiler, Andreas",
    title = "{A Global View of the Off-Shell Higgs Portal}",
    eprint = "1910.04170",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TUM-HEP-1231-19",
    doi = "10.21468/SciPostPhys.8.2.027",
    journal = "SciPost Phys.",
    volume = "8",
    pages = "027",
    year = "2020"
}

@article{Haghighat:2021djz,
    author = "Haghighat, Gholamhossein and Mohammadi Najafabadi, Mojtaba",
    title = "{Search for lepton-flavor-violating ALPs at a future muon collider and utilization of polarization-induced effects}",
    eprint = "2106.00505",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2021"
}

@article{Chen:2021rid,
    author = "Chen, Junmou and Lu, Chih-Ting and Wu, Yongcheng",
    title = "{Measuring Higgs boson self-couplings with 2 \textrightarrow{} 3 VBS processes}",
    eprint = "2105.11500",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP10(2021)099",
    journal = "JHEP",
    volume = "10",
    pages = "099",
    year = "2021"
}

@article{Han:2021lnp,
    author = {Han, Tao and Kilian, Wolfgang and Kreher, Nils and Ma, Yang and Reuter, J\"urgen and Striegl, Tobias and Xie, Keping},
    title = "{Precision test of the muon-Higgs coupling at a high-energy muon collider}",
    eprint = "2108.05362",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY 21-068, PITT-PACC-2110",
    doi = "10.1007/JHEP12(2021)162",
    journal = "JHEP",
    volume = "12",
    pages = "162",
    year = "2021"
}


@article{Qian:2021ihf,
    author = "Qian, Sitian and Li, Congqiao and Li, Qiang and Meng, Fanqiang and Xiao, Jie and Yang, Tianyi and Lu, Meng and You, Zhengyun",
    title = "{Searching for heavy leptoquarks at a muon collider}",
    eprint = "2109.01265",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "9",
    year = "2021"
}

@article{Chiesa:2021qpr,
    author = "Chiesa, Mauro and Mele, Barbara and Piccinini, Fulvio",
    title = "{Multi Higgs production via photon fusion at future multi-TeV muon colliders}",
    eprint = "2109.10109",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "9",
    year = "2021"
}

@article{Buttazzo:2021lzi,
    author = "Buttazzo, Dario and Paradisi, Paride",
    title = "{Probing the muon $g-2$ anomaly with the Higgs boson at a muon collider}",
    doi = "10.1103/PhysRevD.104.075021",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "7",
    pages = "075021",
    year = "2021"
}

@article{Liu:2021akf,
    author = "Liu, Wei and Xie, Ke-Pan and Yi, Zihan",
    title = "{Testing leptogenesis at the LHC and future muon colliders: a $Z'$ scenario}",
    eprint = "2109.15087",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "9",
    year = "2021"
}

@article{Capdevilla:2021kcf,
    author = "Capdevilla, Rodolfo and Curtin, David and Kahn, Yonatan and Krnjaic, Gordan",
    title = "{Systematically Testing Singlet Models for $(g-2)_\mu$}",
    eprint = "2112.08377",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-21-737-T",
    month = "12",
    year = "2021"
}

@article{Chen:2021pqi,
    author = "Chen, Junmou and Li, Tong and Lu, Chih-Ting and Wu, Yongcheng and Yao, Chang-Yuan",
    title = "{The measurement of Higgs self-couplings through $2\rightarrow 3$ VBS in future muon colliders}",
    eprint = "2112.12507",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "12",
    year = "2021"
}

@article{Bandyopadhyay:2021pld,
    author = "Bandyopadhyay, Priyotosh and Karan, Anirban and Mandal, Rusa",
    title = "{Distinguishing signatures of scalar leptoquarks at hadron and muon colliders}",
    eprint = "2108.06506",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IITH-PH-0002/21, SI-HEP-2021-22",
    month = "8",
    year = "2021"
}

@article{Dermisek:2021mhi,
    author = "Dermisek, Radovan and Hermanek, Keith and McGinnis, Navin",
    title = "{Di-Higgs and tri-Higgs boson signals of muon g-2 at a muon collider}",
    eprint = "2108.10950",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.104.L091301",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "9",
    pages = "L091301",
    year = "2021"
}

@article{Sen:2021fha,
    author = "Sen, Chandrima and Bandyopadhyay, Priyotosh and Dutta, Saunak and KT, Aleesha",
    title = "{Displaced Higgs production in Type-III Seesaw at the LHC/FCC, MATHUSLA and Muon collider}",
    eprint = "2107.12442",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IITH-PH-0001/21",
    month = "7",
    year = "2021"
}

@article{Bottaro:2021snn,
    author = "Bottaro, Salvatore and Buttazzo, Dario and Costa, Marco and Franceschini, Roberto and Panci, Paolo and Redigolo, Diego and Vittorio, Ludovico",
    title = "{Closing the window on WIMP Dark Matter}",
    eprint = "2107.09688",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2021"
}

@article{Sahin:2021xzt,
    author = "Sahin, M. and Caliskan, A.",
    title = "{Excited muon production at muon colliders via contact interaction}",
    eprint = "2105.01964",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "5",
    year = "2021"
}

@article{Asadi:2021gah,
    author = "Asadi, Pouya and Capdevilla, Rodolfo and Cesarotti, Cari and Homiller, Samuel",
    title = "{Searching for leptoquarks at future muon colliders}",
    eprint = "2104.05720",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP/5296",
    doi = "10.1007/JHEP10(2021)182",
    journal = "JHEP",
    volume = "10",
    pages = "182",
    year = "2021"
}

@article{Li:2021lnz,
    author = "Li, Tong and Schmidt, Michael A. and Yao, Chang-Yuan and Yuan, Man",
    title = "{Charged lepton flavor violation in light of the muon magnetic moment anomaly and colliders}",
    eprint = "2104.04494",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-021-09569-9",
    journal = "Eur. Phys. J. C",
    volume = "81",
    number = "09",
    pages = "811",
    year = "2021"
}

@article{Bottaro:2021srh,
    author = "Bottaro, Salvatore and Strumia, Alessandro and Vignaroli, Natascia",
    title = "{Minimal Dark Matter bound states at future colliders}",
    eprint = "2103.12766",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP06(2021)143",
    journal = "JHEP",
    volume = "06",
    pages = "143",
    year = "2021"
}

@article{Han:2021udl,
    author = "Han, Tao and Li, Shuailong and Su, Shufang and Su, Wei and Wu, Yongcheng",
    title = "{Heavy Higgs Bosons in 2HDM at a Muon Collider}",
    eprint = "2102.08386",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-2102, ADP-21-2/T1149",
    month = "2",
    year = "2021"
}

@article{Capdevilla:2021fmj,
  author        = {Capdevilla, Rodolfo and Meloni, Federico and Simoniello, Rosa and Zurita, Jose},
  title         = {{Hunting wino and higgsino dark matter at the muon collider with disappearing tracks}},
  eprint        = {2102.11292},
  archiveprefix = {arXiv},
  primaryclass  = {hep-ph},
  reportnumber  = {DESY-21-019, DESY 21-019, IFIC/21-03},
  doi           = {10.1007/JHEP06(2021)133},
  journal       = {JHEP},
  volume        = {06},
  pages         = {133},
  year          = {2021}
}


%%% IMCC Snowmass'21 whitepapers
@article{sm21-imcc-accelerator,
    title={},
    collaboration={International Muon Collider},
    journal={To Appear}
}  

@article{sm21-imcc-physics-3TeV,
    title={The physics case of a 3~TeV muon collider stage},
    collaboration={International Muon Collider},
    journal={To Appear}    
}  

@article{sm21-imcc-physics,
    title={},
    collaboration={International Muon Collider},
    journal={To Appear}    
}  

@article{sm21-imcc-det-technologies,
    title={Promising Technologies and R&D Directions for the Future Muon Collider},
    collaboration={International Muon Collider},
    journal={To Appear}
}  

@article{sm21-imcc-det-perf,
    title={Expected Detector Performance at the Muon Collider},
    collaboration={International Muon Collider},
    journal={To Appear}
}  


